Efficient Sparse-Dense Matrix-Matrix Multiplication on GPUs Using the Customized Sparse Storage Format

Multiplication of a sparse matrix to a dense matrix (SpDM) is widely used in many areas like scientific computing and machine learning. However, existing works under-look the performance optimization of SpDM on modern many-core architectures like GPUs. The storage data structures help sparse matrices store in a memory-saving format, but they bring difficulties in optimizing the performance of SpDM on modern GPUs due to irregular data access of the sparse structure, which results in lower resource utilization and poorer performance. In this paper, we refer to the roofline performance model of GPUs to design an efficient SpDM algorithm called GCOOSpDM, in which we exploit coalescent global memory access, fast shared memory reuse and more operations per byte of global memory traffic. Experiments are evaluated on three Nvidia GPUs (i.e., GTX 980, GTX Titan X Pascal and Tesla P100) with CUDA-8.0 using a large number of matrices including a public dataset and randomly generated matrices. Experimental results show that GCOOSpDM achieves 1.5-8$\times$ speedup over Nvidia's library cuSPARSE in many matrices. We also analyze instruction-level operations on a particular GPU to understand the performance gap between GCOOSpDM and cuSPARSE. The profiled instructions confirm that cuSPARSE spends a lot of time on slow memory access (including DRAM access and L2 cache access), while GCOOSpDM transfers such slow memory access to faster shared memory, which mainly contributes to the performance gain. Results also show that GCOOSpDM would outperform the dense algorithm (cuBLAS) with lower sparsity than cuSPARSE on GPUs.

==> gemm_vs_spdm.tex <==
%\subsection{GEMM vs SpDM}\label{subsection:gemm_vs_spdm}

A naive method to solve SpDM is directly using high-performance GEMM libraries, such as cuBLAS, if the sparsity of matrix A is not very high. High-performance GEMM libraries focus on improving the computational throughput of GPUs. For example, cuBLAS can achieve over 90\% of theoretical peak computational throughput of Nvidia Titan X Pascal. Here we briefly analyze the performance of cuBLAS using the roofline model. Note that we only discuss the square matrix multiplication for simplicity. Generally, for calculation of $\ma{C}=\ma{A} \times \ma{B}$, we need $O(n^3)$ multiplications and additions. Meanwhile, accessing the elements of $\ma{A}$ and $\ma{B}$ is also time consuming in modern GPU architectures. Ideally we need $2 \times n^2$ memory access for $\ma{A}$ and $\ma{B}$ at least. However, due to the limited cache size and registers, practical GEMM implementations have much more main memory access. The previous high-performance GEMM works struggle to reduce the overhead brought by slow memory access and promote the compute core utilization. The optimization principles include [citation]. 

%Thanks to the above memory access optimizations, 

%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.6\linewidth]{cublas_model.pdf}
%	\caption{cuBLAS performance and roofline model.}
%	\label{fig:gpucublas}
%\end{figure} 

However, consider SpDM, in which $\ma{A}$ is of high sparsity. Simply using those high-performance GEMM libraries may bring many useless calculations. Only $1-s$ of $n^3$ calculations have contributions to $\ma{C}$. That is, even high-performance GEMM libraries can achieve nearly peak computational performance of the devices, the effective percentage of those flops is as low as $1-s$. 

\begin{equation}
T = (\alpha n^3+\beta)\times (1-s)
\label{eq:time_sparse}
\end{equation}


